Zero-Shot Monocular Scene Flow Estimation in the Wild

Large models have shown generalization across datasets for many low-level vision tasks, like depth estimation, but no such general models exist for scene flow. Even though scene flow has wide potential use, it is not used in practice because current predictive models do not generalize well. We identify three key challenges and propose solutions for each. First, we create a method that jointly estimates geometry and motion for accurate prediction. Second, we alleviate scene flow data scarcity with a data recipe that affords us 1M annotated training samples across diverse synthetic scenes. Third, we evaluate different parameterizations for scene flow prediction and adopt a natural and effective parameterization. Our resulting model outperforms existing methods as well as baselines built on large-scale models in terms of 3D end-point error, and shows zero-shot generalization to the casually captured videos from DAVIS and the robotic manipulation scenes from RoboTAP. Overall, our approach makes scene flow prediction more practical in-the-wild.

==> figures/figures.tex <==
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{fadings}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{patterns}
\usetikzlibrary{patterns.meta}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{intersections}
\usetikzlibrary{calligraphy}

\definecolor{orangein}{RGB}{247,206,157}
\definecolor{orangeout}{RGB}{229,146,49}
\definecolor{cyanin}{RGB}{155,209,249}
\definecolor{cyanout}{RGB}{69,81,255}
\definecolor{purplein}{RGB}{221,197,235}
\definecolor{purpleout}{RGB}{112,48,160}

\definecolor{darkgray}{RGB}{150,150,150}
\definecolor{verydarkgray}{RGB}{100,100,100}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{verydarkgreen}{RGB}{0,100,0}
\definecolor{darkblue}{RGB}{0,0,150}
\definecolor{darkcyan}{RGB}{0,200,200}
\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkyellow}{RGB}{200,200,0}
\definecolor{darkmagenta}{RGB}{150,0,150}
\definecolor{darkyorange}{RGB}{255,153,15}

\newlength{\range}
\setlength{\range}{100pt}
\newlength{\radius}
\setlength{\radius}{10pt}
\newlength{\tH}
\setlength{\tH}{.15\range}

\newlength{\imW}
\newlength{\imH}


\tikzstyle{currPos}=[
    draw=orangeout,
    fill=orangein,
    style=circle,
    minimum width=\radius,
]

\tikzstyle{startEnd}=[
    draw=purpleout,
    fill=purplein,
    style=circle,
    minimum width=\radius,
]


\tikzstyle{block}=[
    rounded corners,
    align=center,
    inner sep=5pt,
    % minimum width=15pt,
    draw
]


\makeatletter
\pgfdeclareverticalshading{pgf@lib@fade@South}{100bp}{
    color(0bp)=(pgftransparent!100);
    color(25bp)=(pgftransparent!100);
    color(35bp)=(pgftransparent!10);
    color(40bp)=(pgftransparent!0);
    color(100bp)=(pgftransparent!0)}%
\pgfdeclarefading{South}{\pgfuseshading{pgf@lib@fade@South}}%
\makeatother

\makeatletter
\pgfdeclareverticalshading{pgf@lib@fade@North}{100bp}{
    color(0bp)=(pgftransparent!0);
    color(60bp)=(pgftransparent!0);
    color(65bp)=(pgftransparent!10);
    color(75bp)=(pgftransparent!100);
    color(100bp)=(pgftransparent!100)}%
\pgfdeclarefading{North}{\pgfuseshading{pgf@lib@fade@North}}%
\makeatother

==> tables/3d_tracking.tex <==
\begin{table}
    \centering
    \begin{tabular}{lccc}
    \hline
    Methods & ATE$_{3D}$ $\downarrow$ & $\delta_{0.1}$ $\uparrow$ & $\delta_{0.2}$ $\uparrow$ \\
    \hline
    SpaTracker\cite{SpatialTracker} & 0.22 & 0.59 & 0.76 \\
    \hline
    Lifted CoTracker\cite{karaev2023cotracker} & 0.77 & 0.51 & 0.64 \\
    Chained RAFT3D\cite{teed2021raft3d} & 0.70 & 0.12 & 0.25 \\
    \hline
    Chained Ablated Ours & \\    
    \hline
    \end{tabular}
    \caption{
    3D Tracking Evaluation on PointOdyssey Dataset~\cite{zheng2023point}. ATE$_{3D}$ denotes average 3D trajectory error. $\delta_t$ represents percentage of points within $t$ meters of ground truth. 
    }
    \label{table:3d_tracking_results}
    \end{table}

==> tables/experiment_monodepth.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Show not downgrading for Monocular Video Depth Estimation. sota like DepthAnythingV2 here, but would not be as good?
    unimatch\cite{xu2023unimatch},GMFlow\cite{gmflow} not providing metric depth now thus not including.}
    \label{tab:experiment_monodepth}
    \begin{tabular}{l|cc|cc|cc|cc|}
        \hline
        \multirow{2}{*}{Method} 
        & \multicolumn{2}{c|}{VKITTI2\cite{cabon2020vkitti2}} 
        & \multicolumn{2}{c|}{Point-Odyssey\cite{zheng2023point}}         
        & \multicolumn{2}{c|}{Spring\cite{Mehl2023_Spring}} 
        & \multicolumn{2}{c|}{DynamicReplica\cite{karaev2023dynamicstereo}} 
        \\
        & AbsRel$\downarrow$ & $\delta$1$\uparrow$ 
        & AbsRel$\downarrow$ & $\delta$1$\uparrow$ 
        & AbsRel$\downarrow$ & $\delta$1$\uparrow$  \\
        \hline
        DepthAnythingV2\cite{depth_anything_v2} \\
        \midrule
        self-mono-sf (ours) & 0.32 & 0.458 \\ 
        \midrule
        MASt3R\cite{mast3r}  & 0.32 & 0.432 \\
        \midrule
        Ablated Ours - trained on SHIFT-only & 0.15 & 0.907  \\
        Ablated Ours - trained on DynamicReplica+SHIFT & 0.13 & 0.906\\
        \hline
    \end{tabular}
\end{table*}

==> tables/experiment_nvs.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Generalizable Scene-Level Dynamic Novel View Synthesis given Monocular Input. 
    Follow the setting of the only closest prior work pgdvs (did not optimize for appearance).}
    \label{tab:experiment_nvs}
    \setlength{\tabcolsep}{1pt}
        \begin{tabular}{|l|ccc|ccc|}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{NVIDIA Dynamic Scenes\cite{NVIDIAdataset}} & \multicolumn{3}{c|}{DyCheck iPhone\cite{gao2022dycheck}} \\
        \cline{2-7}
     & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS$\times1000$ $\downarrow$ 
     & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
        \hline
        pgdvs\cite{zhao2024pgdvs} & 26.15 & 0.922 & 64.29 & 15.88 &  0.548 & 0.340\\
        \hline
        Flash3D\cite{szymanowicz2024flash3d}+RAFT & \\
        \hline
        Ablated Ours &     \\
        \hline
    \end{tabular}
\end{table*}

==> tables/experiment_opticalflow.tex <==
\begin{table*}[htbp]
    \centering
    \caption{(Optional)Comparison of Methods across Datasets and Metrics for Optical Flow Prediction (in-domain, out-domain order might change)}
    \label{tab:experiment_opticalflow}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
        \hline
        \multirow{3}{*}{Method} & \multicolumn{6}{c|}{In-Domain} & \multicolumn{6}{c}{Out-Domain} \\
        \cline{2-13}
        & \multicolumn{2}{c|}{DynamicReplica\cite{karaev2023dynamicstereo}} 
        & \multicolumn{2}{c|}{VKITTI2\cite{cabon2020vkitti2}} 
        & \multicolumn{2}{c|}{KITTI\cite{cabon2020vkitti2}} 
        & \multicolumn{2}{c|}{Sintel\cite{Mehl2023_Spring}} 
        & \multicolumn{2}{c|}{Spring\cite{Mehl2023_Spring}} 
        & \multicolumn{2}{c}{SceneFlow\cite{Mayer_2016_CVPR}} \\
        & Metric 1 & Metric 2 & Metric 1 & Metric 2 & Metric 1 & Metric 2 & Metric 1 & Metric 2 & Metric 1 & Metric 2 & Metric 1 & Metric 2 \\
        \hline
        ... \\
        RAFT\cite{} & & & & & & & & & & & \\
        RAFT-3D\cite{teed2021raft3d} & & & & & & & & & & & \\
        SEA-RAFT\cite{wang2024sea} & & & & & & & & & & &  \\
        \midrule
        CamliFlow\cite{liu2022camliflow} & & & & & & & & & & &  \\
        CamLiRAFT\cite{liu2023learning} & & & & & & & & & & & \\
        CamLiRAFT-L\cite{liu2023learning} & & & & & & & & & &  & \\
        \midrule
        GMFlow\\
        UniMatch\\
        \midrule
        Ablated Ours & & & & & & & & & &   \\
        \hline
    \end{tabular}
\end{table*}

==> tables/experiment_sceneflow.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Comparison of Methods across Datasets and Metrics for Monocular Scene Flow Prediction (in-domain, out-domain order might change)
    Search for Kitti benchmark monocular scene flow; think about chaining; see recent work's dataset}
    \label{tab:experiment_sceneflow}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{l|cc|cc|cc|cc}
        \hline
        \multirow{3}{*}{Method} & \multicolumn{4}{c|}{In-Domain} & \multicolumn{4}{c}{Out-Domain} \\
        \cline{2-9}
        & \multicolumn{2}{c|}{VKITTI2\cite{cabon2020vkitti2}} 
        & \multicolumn{2}{c|}{KITTI\cite{cabon2020vkitti2}}
        & \multicolumn{2}{c|}{Spring\cite{Mehl2023_Spring}} 
        & \multicolumn{2}{c}{SceneFlow\cite{Mayer_2016_CVPR}} 
        \\ & Metric 1 & Metric 2 
        & Metric 1 & Metric 2 
        & Metric 1 & Metric 2 
        & Metric 1 & Metric 2\\
        \hline
        self-mono-sf... \\
        optical expansion + single image depth \\
        RAFT-3D\cite{teed2021raft3d} & & & & & & & & \\
        \midrule
        CamliFlow\cite{liu2022camliflow} & & & & & & & & \\
        CamLiRAFT\cite{liu2023learning} & & & & & & & & \\
        CamLiRAFT-L\cite{liu2023learning} & & & & & & & & \\
        \midrule
        DUSt3R\cite{dust3r}+RAFT  & & & & & & & & \\
        MASt3R\cite{mast3r}+RAFT  & & & & & & & & \\
        \midrule
        Ablated Ours  & & & & & & & & \\
        \hline
    \end{tabular}
\end{table*}

==> tables/monocular_scene_flow_kitti.tex <==
\begin{table*}
    \centering
    \begin{tabular}{|l|cccc|cccc|}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{4}{c|}{KITTI Scene Flow Training Set} & \multicolumn{4}{c|}{KITTI Scene Flow Testing Set} \\
    \cline{2-9}
     & D1-all $\downarrow$ & D2-all $\downarrow$ & F1-all $\downarrow$ & SF-all $\downarrow$ & D1-all $\downarrow$ & D2-all $\downarrow$ & F1-all $\downarrow$ & SF-all $\downarrow$ \\
    \hline
    GeoNet\cite{geonet} & 49.54 & 58.17 & 37.83 & 71.32 & - & - & - & - \\
    DF-Net\cite{dfnet} & 46.50 & 61.54 & 27.47 & 73.30 & - & - & - & - \\
    EPC++\cite{EPC++} & 23.84 & 60.32 & 19.64 & - & - & - & - & - \\
    Self-Mono-SF\cite{Hur:2020:SSM} & 31.25 & 34.86 & 23.49 & 47.05 & 34.02 & 36.34 & 23.54 & 49.54 \\
    Self-Mono-SF (results) & 30.48 & 34.38 & 23.06 & 46.33 \\
    Self-Mono-SF (ours) & 48.64 & 64.32 & 91.37 & 96.80  \\
    DRAFT\cite{draft} & 26.41 & 28.89 & 18.71 & 37.58 & - & - & - & - \\
    Multi-Mono-SF\cite{Hur:2021:SSM} & 27.33 & 30.44 & 18.92 & 39.82 & 30.78 & 34.41 & 19.54 & 44.04 \\
    RAFT-MSF\cite{raftmsf} & 18.34 & 23.65 & 17.51 & 30.97 & 21.21 & 27.51 & 18.37 & 34.98 \\
    EMR-MSF\cite{emrmsf} & 8.37 & 12.86 & 11.58 & 18.11 & 9.70 & 14.51 & 11.93 & 19.74 \\
    \hline
    MASt3R\cite{mast3r}+RAFT - Pretrained MASt3R + KITTI RAFT (not finetuned) & 96.23 & - & 6.14 & - \\
    MASt3R\cite{mast3r}+RAFT - Pretrained MASt3R + Pretrained RAFT (not finetuned) & 96.23 & - & 16.51 & - \\
    \hline
    Ablated Ours - trained on Kubric-movif-decomposed (flow2d-only) & 99.64 & 95.74 & 64.07 & 99.94 \\
    Ablated Ours - trained on VKITTI2-decomposed & 23.15 & 28.93 & 45.68 & 55.92 \\
    Ablated Ours - trained on DynamicReplica+SHIFT (depth-only) & 74.61 & - & - & - \\
    Ablated Ours - trained on DynamicReplica+SHIFT & 71.31 & 58.66 & 68.55 & 84.73 \\
    \hline
    \end{tabular}
    \caption{
    Monocular scene flow evaluation on KITTI 2015\cite{Menze2015ObjectSF} Training set and Testing set. 
    Numbers adopted from each paper. Not the foreground-only version.
    Mono-SF\cite{monosf}, OpticalExpansion\cite{yang2020upgrading} and BinaryTTC\cite{binaryttc} not included as numbers are not ready.}
    \label{tab:monocular_scene_flow_kitti}
    \end{table*}

==> tables/monocular_scene_flow_ours.tex <==
\begin{table*}
    \centering
    \begin{tabular}{|l|cccc|cccc|}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{4}{c|}{Virtual KITTI 2\cite{cabon2020vkitti2}}  & \multicolumn{4}{c|}{Spring\cite{Mehl2023_Spring}} \\
    \cline{2-9}
    & D1-all $\downarrow$ & D2-all $\downarrow$ & F1-all $\downarrow$ & SF-all $\downarrow$ & D1-all $\downarrow$ & D2-all $\downarrow$ & F1-all $\downarrow$ & SF-all $\downarrow$ \\
    \hline
    self-Mono-SF (ours) & 74.96 & - & 86.40 & -\\
    \hline
    MASt3R\cite{mast3r}+RAFT(kitti) & 57.07 & - & 2.23 & - \\
    \hline
    Ablated Ours - trained on SHIFT-only & 37.10 & - & 24.57 & - \\
    Ablated Ours - trained on DynamicReplica+SHIFT & 33.02 & - & 24.66 & - \\
    Ablated Ours - trained on VKITTI2-decomposed & 3.80 & - & 20.69 & - \\
    \hline
    \end{tabular}
    \caption{Monocular scene flow evaluation on Spring Dataset\cite{Mehl2023_Spring} and VirtualKITTI2 dataset\cite{cabon2020vkitti2}.
    Spring dataset has leaderboard, but only stereo results. VKITTI2 did not provide scene flow protocol. Select all variants of Scene06 for evaluation. We use Left Cameras for both.
    DUSt3R / MASt3R trained on the same set as well ablated?
    }
    \label{tab:monocular_scene_flow_ours}
    \end{table*}
